Nucleosynthesis and CMB bounds on photophilic ALPs: a fresh look

We provide a fresh look at the cosmological constraints on axion-like particles (ALPs) that couple predominantly to photons, focusing on lifetimes $\tau_{a} \lesssim 10^{4}\, {\rm s}$ and masses $m_a\lesssim 10\,{\rm GeV}$. We consider Big Bang Nucleosynthesis (BBN) and Cosmic Microwave Background (CMB) bounds and explore how these limits depend upon the unknown reheating temperature of the Universe, $T_{\rm reh}$. Compared with some previous studies, we account for the rare decays of these ALPs into light hadrons and show that this leads to extended constraints for several reheating temperatures. Our limits are cast in a model-independent way, and we identify regions of parameter space where these ALPs could alleviate small tensions in the determinations of $N_{\rm eff}$ and the deuterium abundance.

==> header.tex <==
\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

\usepackage{eso-pic}
\newcommand{\reportnum}[2]{
  \AddToShipoutPictureBG*{%
    \AtPageUpperLeft{%
      \hspace{0.75\paperwidth}%
      \raisebox{#1\baselineskip}{%
        \makebox[0pt][l]{\textnormal{#2}}
  }}}%
}

\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{graphicx,tabularx}
\usepackage{color}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage{multirow}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{cleveref}
\usepackage{slashed}
\usepackage[normalem]{ulem}
\usepackage{scalerel}
\usepackage{fontawesome5}
\usepackage{textgreek}

\setlist[description]{leftmargin=0.3cm}
\setlist[itemize]{leftmargin=0.5cm}

\newcommand{\be}{\begin{equation} \begin{aligned}}
\newcommand{\ee}{\end{aligned} \end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

\def\figureautorefname~#1\null{Fig.\,#1\null}
\def\tableautorefname~#1\null{Tab.\,#1\null}
\renewcommand{\sectionautorefname}{Sec.}
\renewcommand{\subsectionautorefname}{Sec.}
\def\equationautorefname~#1\null{Eq.\,(#1)\null}

% General symbols
\newcommand{\im}{\mathrm{i}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eg}{{e.\,g.}~}
\newcommand{\ie}{{i.\,e.}~}
\newcommand{\equivalent}{\simeq}
\newcommand{\br}{\mathrm{BR}}

% Units
\usepackage{siunitx}
\sisetup{separate-uncertainty  = true,
         print-unity-mantissa = false,
         exponent-product      = \cdot,
         range-phrase = \text{--},
         range-units  = single
}

\newcommand{\neff}{\ensuremath{N_{\rm eff}}\xspace}
\newcommand{\dH}{\ensuremath{\text{D}/\text{H}|_{\rm P}}\xspace}
\newcommand{\mev}{\ensuremath{\,{\rm MeV}}\xspace}
\newcommand{\yp}{\ensuremath{Y_{\rm P}}\xspace}
\newcommand{\gev}{\ensuremath{\,{\rm GeV}}\xspace}
\newcommand{\tev}{\ensuremath{\,{\rm TeV}}\xspace}
\newcommand{\s}{\ensuremath{\,{\rm s}}\xspace}
\newcommand{\dneff}{\ensuremath{\Delta N_{\text{eff}}}\xspace}
\newcommand{\pn}{\ensuremath{p\leftrightarrow n}\xspace}
\newcommand{\Treh}{\ensuremath{T_{\rm reh}}\xspace}

\newcommand{\ab}{\text{ab}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\pb}{\text{pb}}
\newcommand{\ipb}{\text{pb}^{-1}}

\newcommand{\nm}{\text{nm}}
\newcommand{\micm}{\mu\text{m}}
\newcommand{\mm}{\text{mm}}
\newcommand{\cm}{\text{cm}}
\newcommand{\m}{\text{m}}
\newcommand{\km}{\text{km}}

\newcommand{\mrad}{\text{mrad}}
\newcommand{\murad}{\mu\text{rad}}

\newcommand{\g}{\text{g}}
\newcommand{\kg}{\text{kg}}
\newcommand{\ton}{\text{t}}
\newcommand{\sr}{\text{sr}}
\newcommand{\ns}{\text{ns}}

\newcommand{\fasernu}{FASER$\nu$~}

%comments
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}
%\newcommand{\changed}[2]{#2}
\newcommand{\Felix}[1]{\textcolor{magenta}{[FK: #1]}}
\newcommand{\st}[1]{\textcolor{blue}{[ST: #1]}}

\crefname{section}{Sec.}{Secs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{table}{Table}{Tables}
\crefname{equation}{Eq.}{Eqs.}
\crefname{appendix}{Appendix}{Appendices}

%Ref Style
\bibliographystyle{utphys}

